Additive Decoders for Latent Variables Identification and Cartesian-Product Extrapolation

We tackle the problems of latent variables identification and ``out-of-support'' image generation in representation learning. We show that both are possible for a class of decoders that we call additive, which are reminiscent of decoders used for object-centric representation learning (OCRL) and well suited for images that can be decomposed as a sum of object-specific images. We provide conditions under which exactly solving the reconstruction problem using an additive decoder is guaranteed to identify the blocks of latent variables up to permutation and block-wise invertible transformations. This guarantee relies only on very weak assumptions about the distribution of the latent factors, which might present statistical dependencies and have an almost arbitrarily shaped support. Our result provides a new setting where nonlinear independent component analysis (ICA) is possible and adds to our theoretical understanding of OCRL methods. We also show theoretically that additive decoders can generate novel images by recombining observed factors of variations in novel ways, an ability we refer to as Cartesian-product extrapolation. We show empirically that additivity is crucial for both identifiability and extrapolation on simulated data.

==> logs.tex <==
We now present empirical validations of the theoretical results presented earlier. To achieve this, we compare both additive and non-additive decoders at their ability to both identify ground-truth latent factors (Theorems~\ref{thm:local_disentanglement} \& \ref{thm:local2global}) and extrapolate (Corollary~\ref{cor:extrapolation}) when trained to solve the reconstruction task on simple \seb{(64x64x3)} images consisting of two balls resting in space. We consider two datasets: one where the two ball positions can only vary along the $y$-axis (\textbf{ScalarLatents}) and one where the positions can vary along both the $x$ and $y$ axes (\textbf{BlockLatents}). 

\textbf{ScalarLatents:} The ground-truth latent vector $\vz = (\vz_1, \vz_2)$ corresponds to the height of both balls and thus the partition is simply $\gB = \{\{1\}, \{2\}\}$ (each object has only one latent factor). This simple setting is interesting to study since the low dimensionality of the latent space ($d_z = 2$) allows for exhaustive visualizations like Figure~\ref{fig:extrapolation-exps}. To study Cartesian-product extrapolation (Corollary~\ref{cor:extrapolation}), we sample the latent factor $\vz$ uniformly from the L-shaped support given by $\gZ^\train := [0,1] \times [0,1] \setminus [0.5,1] \times [0.5,1] $. This means the training set does not contain images where both balls appear in the upper half of the image. 

\textbf{BlockLatents:} The ground-truth latent vector $\vz = (\vz_1, \vz_2, \vz_3, \vz_4)$ corresponds to the $xy$ positions of both balls where the partition is simply $\gB = \{\{1, 2\}, \{3, 4\}\}$ (each object has two latent factors). Thus, this more challenging setting illustrates ``block-disentanglement''. The latent $\vz$ is sampled uniformly from the hypercube $[0,1]^4$ but the images presenting occlusion (when a ball is behind another) are rejected from the dataset. We discuss how additive decoders cannot model images presenting occlusion in Appendix~\ref{app:occlusion}. 

\subsection{Two balls experiments}
\begin{itemize}
    \item \textbf{Show disentanglement:} On the ``square-shaped'' support, show disentanglement is possible with additive decoders, but not with non-additive decoders (even if they have similar reconstruction scores). Might also want to add another experiment with a disk-shaped support. Table~\ref{tab:extrapolate_basic} Figure~\ref{fig:violin_plot}
    \item \textbf{Show extrapolation:} On the ``L-shaped'' support, show additive decoders can extrapolate, but non-additive decoders cannot.

    \divyat{The above two points have been done for multiple seeds and verify our theory. Next steps; use baseline like BetaVAE and show they fail either due to non-additive decoder or dependencies in the latent space.}

    \item \textbf{Show importance of having enough samples, since with too few samples, we get problems that resemble having a disconnected support.}

    \divyat{TODO: We already have evidence for increase in performance from 10k to 50k training samples. Lets increase till 100k and make a plot comparing the performance of additive and base decoder.}
   
    \item \textbf{Show importance of having a connected support} Switch in permutation? Non-monotonous relation between $\vz$ and $\hat\vz$?

    \divyat{Done; the results show much less MCC as compared to the connected support case. We do not observe a switch permutation but indeed observe the non-monotonous relationship between inferred and true latents.}
    
    \item \textbf{Demonstrate usefulness of further training the encoder} Show extrapolation of encoder is possible only with this procedure.

    \divyat{The above point might not be needed since the MCC on extrapolated dataset is already considerably higher than baselines; perhaps because of the simplicity of our dataset and we can refer to this for future work on more complicated datasets.}
    
\end{itemize}

\subsection{Disentanglement for multiple balls experiments (Or maybe a version of multiple digit MNIST?)}

\begin{itemize}
    \item Idea is to show disentanglement for multiple balls moving in xy directions. This is important to show case block disentanglement. And also this is a toy experiment that represents broad class of problems...

    \divyat{Basic check has been done that shows we need increased latent dimension for good reconstruction. TODO: Check with multiple seeds for both independent and dependent latent cases and compute the block MCC metric.}
    
\end{itemize}

\subsection{3D Shapes}

For this set of experiments, we might have to keep the factors "camera-angle" and "object shape" fixed, since they are not ``additive''. We can try both with and without to showcase the importance of the data satisfying the assumption of our data-generating process.

\begin{itemize}
    \item \textbf{Show disentanglement}
    \item \textbf{Show extrapolation}
    \item \textbf{Demonstrate our procedure to train encoder on generated images.}
\end{itemize}

\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c}
        \toprule
         Case & AE Base & AE Additive \\
         \midrule
          In Distribution & $82.6 \pm 4.59$  & $94.5 \pm 3.53$ \\           
         \hline
         OOD Distribution &  $78.7 \pm 6.20$ &  $94.3 \pm 4.63$ \\            
         \bottomrule
    \end{tabular}
    \caption{Extrapolation experiments with balls moving along y-axis only (Old results with smaller model capactity)}
    \label{tab:extrapolate_basic}
\end{table}


\begin{figure}
    \centering
    \includegraphics[scale=0.25]{figures/Non_Block_In_Support.pdf}
    \caption{'In Support'}
    \label{fig:my_label}
    \includegraphics[scale=0.25]{figures/Non_Block_OOD_Support.pdf}
    \caption{'OOD Support'}
    \label{fig:violin_plot}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/additive_decoder/latent_support_seed_median.jpg}
    \includegraphics[scale=0.22]{figures/additive_decoder/traversed_image_seed_median.jpg}
    \caption{Additive Decoder}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/base_decoder/latent_support_seed_median.jpg}
    \includegraphics[scale=0.22]{figures/base_decoder/traversed_image_seed_median.jpg}
    \caption{Base Decoder}
    \label{fig:my_label}
\end{figure}


\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c}
        \toprule
         Case & AE Base & AE Additive \\
         \midrule
         IID Latent & $671.5 \pm 131.55$  & $812.4 \pm 261.8$ \\           
         \hline
         SCM Latent & $381.7 \pm 145.95$ &  $348.7 \pm 170.24$ \\            
         \bottomrule
    \end{tabular}
    \caption{Recon: Block disentanglement}
    \label{tab:block-disentangle}
    
    \begin{tabular}{c|c|c}
        \toprule
         Case & AE Base & AE Additive \\
         \midrule
         IID Latent & $70.3 \pm 5.53$  & $91.1 \pm 4.28$ \\           
         \hline
         SCM Latent & $88.6 \pm 2.06$ &  $99.9 \pm 0.01$ \\            
         \bottomrule
    \end{tabular}
    \caption{MCC: Block disentanglement}
    \label{tab:block-disentangle}
\end{table}

\begin{table}[th]
    \centering
    \begin{tabular}{c|c|c}
        \toprule
         Case & AE Base & AE Additive \\
         \midrule
         IID Latent & $618.94 \pm 97.4$  & $811.1 \pm 262.4$ \\           
         \hline
         SCM Latent & $48834.48 \pm 1239.15$ &  $43316.5 \pm 3720.97$ \\            
         \bottomrule
    \end{tabular}
    \caption{Recon: Block disentanglement; Cross Eval}
    \label{tab:block-disentangle}
    
    \begin{tabular}{c|c|c}
        \toprule
         Case & AE Base & AE Additive \\
         \midrule
         IID Latent & $85.8 \pm 2.88$  & $96.5 \pm 1.75$ \\           
         \hline
         SCM Latent & $ 64.9 \pm 2.12 $ &  $85.4 \pm 2.01$ \\            
         \bottomrule
    \end{tabular}
    \caption{MCC: Block disentanglement; Cross Eval}
    \label{tab:block-disentangle}
\end{table}



